CARL: Congestion-Aware Reinforcement Learning for Imitation-based Perturbations in Mixed Traffic Control

Human-driven vehicles (HVs) exhibit complex and diverse behaviors. Accurately modeling such behavior is crucial for validating Robot Vehicles (RVs) in simulation and realizing the potential of mixed traffic control. However, existing approaches like parameterized models and data-driven techniques struggle to capture the full complexity and diversity. To address this, in this work, we introduce CARL, a hybrid approach that combines imitation learning for close proximity car-following and probabilistic sampling for larger headways. We also propose two classes of RL-based RVs: a safety RV focused on maximizing safety and an efficiency RV focused on maximizing efficiency. Our experiments show that the safety RV increases Time-to-Collision above the critical 4-second threshold and reduces Deceleration Rate to Avoid a Crash by up to 80%, while the efficiency RV achieves improvements in throughput of up to 49%. These results demonstrate the effectiveness of CARL in enhancing both safety and efficiency in mixed traffic.

==> sections/prelim.tex <==
\section{Preliminaries} 
\label{sec:prelim}
% In this section, we introduce the Intelligent driver model as well as various approaches used by Robot Vehicles (RV) for traffic flow control.
% Various robot vehicles (RV), described in section~\ref{subsec:controllers} with stabilization characteristics are presented in Table~\ref{table:controllers}, have been developed to prevent the formation of stop-and-go traffic. 
% We briefly introduce IDM, \h{various RVs considered in this study, and the problem formulation for RL}. 

% \subsection{Reinforcement Learning (RL)}
% RL is a $T$-step episodic task where an agent interacts with its environment and seeks to maximize the sum of discounted rewards. At each time step, the agent is given a state $s$, responds with an action $a$, and then the environment returns the next state $s'$ and reward $r$. This is formalized as a partially observable markov decision process represented as \((\mathcal{S}, \mathcal{A}, \mathcal{P}, \mathcal{R}, \Omega, \mathcal{O}, \gamma)\), where \(\mathcal{S}\) represents the set of states, \(\mathcal{A}\) is the set of actions, \(\mathcal{P}(s', r | s, a)\) describes the environment dynamics, \(\mathcal{R}(s,a)\) is the reward function, \(\Omega\) represents the set of observations, \(\mathcal{O}(o | s', a)\) is the observation function defining the probability of observing \(o\) given the action \(a\) has led to state \(s'\), and \(\gamma\) is the discount factor. RL-based methods have gained popularity as an effective alternative to model-based or heuristic-based methods. 

